The Simple Economics of Approximately Optimal Auctions

The intuition that profit is optimized by maximizing marginal revenue is a guiding principle in microeconomics. In the classical auction theory for agents with linear utility and single-dimensional preferences, Bulow and Roberts (1989) show that the optimal auction of Myerson (1981) is in fact optimizing marginal revenue. In particular Myerson's virtual values are exactly the derivative of an appropriate revenue curve. This paper considers mechanism design in environments where the agents have multi-dimensional and non-linear preferences. Understanding good auctions for these environments is considered to be the main challenge in Bayesian optimal mechanism design. In these environments maximizing marginal revenue may not be optimal and there is sometimes no direct way to implement the marginal revenue maximization. Our contributions are three fold: we characterize the settings for which marginal revenue maximization is optimal (by identifying an important condition that we call revenue linearity), we give simple procedures for implementing marginal revenue maximization in general, and we show that marginal revenue maximization is approximately optimal. Our approximation factor smoothly degrades in a term that quantifies how far the environment is from ideal (where marginal revenue maximization is optimal). Because the marginal revenue mechanism is optimal for single-dimensional agents, our generalization immediately approximately extends many results for single-dimensional agents. One of the biggest open questions in Bayesian algorithmic mechanism design is developing methodologies that are not brute-force in the size of the agent type space. Our methods identify a subproblem that, e.g., for unit-demand agents with values drawn from product distributions, enables approximation mechanisms that are polynomial in the dimension.

==> DPST.tex <==
\section{Proofs in \autoref{sec:nonmonotone}}
\label{sec:DPST}

\begin{proof}[Proof of Theorem~\ref{thm:majorize}]

% In this section we give a proof to Theorem~\ref{thm:majorize}.  
The essence of the proof can be seen as a
Birkhoff-von~Neumann-Rado style decomposition to a vector by another one majorizing it.  However, due to the
discreteness of the type space, extra care need be taken.  We start from the following definition, .

% \newcommand{\DPST}{DPST}
\begin{definition}[Distribution Preserving Stochastic Transformation (DPST)]
\label{def:smap}%
A pair of functions $(\pi_i, \mu_i)$, $\pi_i,\mu_i : T_i \times T_i \to [0,1]$ is called a \emph{``stochastic
transformation''} for agent $i$, if{f} for all $\Tp \in T_i$, $\sum_{\Tp' \in T_i} \pi_i(\Tp', \Tp) = 1$. A stochastic
transformation can be applied to agent $i$ by replacing agent $i$ with a proxy that does the following. If the actual type
reported by agent $i$ is $t_i$, the proxy instead reports a type $t'_i=\Pi_i(t_i)$ where $\Pi_i(t_i)$ is a random function that
returns each $\Tp' \in T_i$ with probability $\pi_i(\Tp', t_i)$. If the proxy is chosen as a winner, then the proxy announces
agent $i$ as a winner with probability $\mu_i(t'_i, t_i)$, otherwise agent $i$ is not a winner. Furthermore,
A stochastic transformation $(\pi_i, \mu_i)$ is
called \emph{``distribution preserving''} iff for all $\Tp' \in T_i$, $\sum_{\Tp \in T_i} \pi_i(\Tp', \Tp) f_i(\Tp) = f_i(\Tp')$,
i.e., the the distribution of the types reported by the proxy is the same as the distribution of types of the actual agent $i$.
We use the notation $(\pi_i, \mu_i) \times \Inter{x}_i$ to denote the new interim allocation rule that results from applying
$(\pi_i, \mu_i)$ to $\Inter{x}_i$.
\end{definition}

Note that for any given ex-post allocation rule $x : T \to [0,1]$, applying a \DPST{}  $(\pi_i, \mu_i)$ to some agent $i$ yields
a new feasible ex-post allocation rule in which all the agents, except for agent $i$, observe the same interim allocation rules
as before. We will show that by carefully choosing $(\pi_i, \mu_i)$ we can convert $\Inter{x}_i$ to any other interim allocation
rule $\Inter{x}'_i$ given that $\Inter{x}'_i \preceq \Inter{x}_i$.

\begin{theorem}
\label{thm:smap} Given any two interim allocation rules $\Inter{x}_i$ and $\Inter{x}^*_i$ such that $\Inter{x}_i \succeq
\Inter{x}^*_i$, there exists a \DPST{} $(\pi_i, \mu_i)$ such that $\Inter{x}^*_i = (\pi_i, \mu_i)\times \Inter{x}_i$.
\end{theorem}

We prove the previous theorem by showing that there is sequence of \DPST{}s that can be applied to $\Inter{x}_i$ to obtain
$\Inter{x}^*_i$. We first show that any such sequence can be converted to a single \DPST{}.

\begin{lemma}
Any sequence of two or more \DPST{}s can be substituted by an equivalent \DPST.
\end{lemma}
\begin{proof}
Let $(\pi_i, \mu_i)$ and $(\pi'_i, \mu'_i)$ be two \DPST{}s. We define $(\pi''_i, \mu''_i) = (\pi_i, \mu_i) \times (\pi'_i,
\mu'_i)$ as follows.
\begin{align*}
    \forall \Tp, \Tp'' \in T_i: \qquad \pi''_i(\Tp'',\Tp) &=
        \sum_{\Tp' \in T_i} \pi_i(\Tp'',\Tp')\cdot \pi'_i(\Tp',\Tp) \\
    \forall \Tp, \Tp'' \in T_i: \qquad \mu''_i(\Tp'',\Tp) &=
        \sum_{\Tp' \in T_i} \mu_i(\Tp'',\Tp')\cdot \mu'_i(\Tp',\Tp)
\end{align*}
It is easy to see that for any $\Inter{x}_i$, $(\pi_i, \mu_i) \times \left((\pi'_i, \mu'_i) \times \Inter{x}_i\right) = (\pi''_i,
\mu''_i) \times \Inter{x}_i$.
\end{proof}

Next, we describe three kinds of \DPST{} that we will use later. All of the following \DPST{}s take an initial allocation
$\Inter{x}_i$ as one of their arguments and assume that $T_i=\{\Tp_i^1, \Tp_i^2, \cdots \}$ is a relabeling of types in
decreasing order of $\Inter{x}_i$, and $F_i^j = \sum_{r=1}^{j} f_i(\Tp_i^r)$. Each one of them returns a \DPST{} $(\pi_i, \mu_i)$
that can be be applied to $\Inter{x}_i$ to achieve a certain effect.
\begin{itemize}
\item $\ReorderTypes(\Inter{x}_i, \{{\Tp^*}_i^1, {\Tp^*}_i^2, \cdots \})$.
Given an interim allocation rule $\Inter{x}_i$ and an ordering of types of agent $i$, i.e., ${\Tp^*}_i^1, {\Tp^*}_i^2, \cdots $,
this \DPST{} converts $\Inter{x}_i$ to another interim allocation rules that gives the highest probability of allocation to
${\Tp^*}_i^1$, then to ${\Tp^*}_i^2$, and so on. Let ${F^*}_i^j = \sum_{r=1}^{j} f_i({\Tp^*}_i^r)$. This \DPST{} can be described
as follows. If agent $i$ reports a type $t_i={\Tp}_i^{j^*}$, then the proxy chooses $Z$ uniformly at random from the interval
$[{F^*}_i^{j^*-1},{F^*}_i^{j^*})$, and finds the index $j'$ such that $Z \in [{F}_i^{j'-1}, {F}_i^{j'})$. The proxy reports $t'_i
= {\Tp}_i^{j'}$. The agent wins whenever the proxy wins. Formally, $(\pi_i, \mu_i)$ can be defined as
\begin{align*}
    \forall j', j^* \in [|T_i|]: \qquad \pi_i(\Tp_i^{j'},{\Tp^*}_i^{j^*}) &= \left| [{F}_i^{j'-1},{F}_i^{j'}) \cap [{F^*}_i^{j^*-1},{F^*}_i^{j^*})  \right| \\
    \forall j', j^* \in [|T_i|]: \qquad \mu_i(\Tp_i^{j'},{\Tp^*}_i^{j^*}) &= 1
\end{align*}

\item $\LowerTypes(\Inter{x}_i, a)$.
This \DPST{} tries to zero the the interim allocation probability for all types $\Tp_i^j$ such that $j \ge a$ as explained next.
If agent $i$ reports a type $t_i={\Tp}_i^j$, then the proxy reports the same type, i.e., $t'_i=\Tp_i^j$. The agent wins iff $j <
a$ and the proxy wins. Formally, $(\pi_i, \mu_i)$ can be defined as
\begin{align*}
    \forall j, j' \in [|T_i|]: \qquad \pi_i(\Tp_i^{j'},\Tp_i^j) &=
        \begin{cases}
            1 & j = j' \\
            0 & j \neq j'
        \end{cases} \\
    \forall j, j' \in [|T_i|]: \qquad \mu_i({\Tp}_i^{j'},\Tp_i^j) &=
        \begin{cases}
            1 & j < a \\
            0 & j \ge a
        \end{cases} \\
\end{align*}

\item $\MixTypes(\Inter{x}_i, a, b)$.
This \DPST{} mixes the types in range $\Tp_i^a,\cdots, \Tp_i^b$ uniformly as explained next. If agent $i$ reports a type
$t_i=\Tp_i^j$, then if $j \not \in a\cdots b$ the proxy reports the same type $t'_i=\Tp_i^j$, otherwise the proxy chooses $Z$
uniformly at random from the interval $[{F}_i^{a-1},{F}_i^b)$ and finds $j'$ such that $Z \in [F_i^{j'-1},F_i^{j'})$. The proxy
reports $t'_i = {\Tp}_i^{j'}$. The agent wins whenever the proxy wins. Formally, $(\pi_i, \mu_i)$ can be defined as
\begin{align*}
    \forall j, j' \in [|T_i|]: \qquad \pi_i({\Tp}_i^{j'},\Tp_i^j) &=
    \begin{cases}
    \frac{F_i^{j'}-F_i^{j'-1}}{{F}_i^b-{F}_i^{a-1}} & a \le j \le b \\
    1   & \text{otherwise}
    \end{cases}
     \\
    \forall j, j' \in [|T_i|]: \qquad \mu_i({\Tp}_i^{j'},\Tp_i^j) &= 1
\end{align*}
\end{itemize}

Next, we present an algorithm that can convert any interim allocation rule $\Inter{x}_i$ to any other interim allocation rule
$\Inter{x}^*_i$ by combining a sequence of the \DPST{}s described above, given that $\Inter{x}^*_i \preceq \Inter{x}_i$.

\begin{algorithm}
\textbf{Input:} Two interim allocation rules $\Inter{x}_i$ and $\Inter{x}^*_i$. Let $T_i=\{{\Tp^*}_i^1, {\Tp^*}_i^2, \cdots \}$
denote a relabeling of types in decreasing order of $\Inter{x}^*_i$. Also let ${F^*}_i^j = \sum_{r=1}^{j} f_i({\Tp^*}_i^r)$. \\
\textbf{Output:} A \DPST{} that converts $\Inter{x}_i$ to $\Inter{x}^*_i$.
\begin{algorithmic}[1]
    \STATE Let $(\pi^{(0)}_i, \mu_i^{(0)}) \leftarrow \ReorderTypes({\Inter{x}_i}, \{{\Tp^*}_i^1, {\Tp^*}_i^2, \cdots \})$.
    \STATE Let $\Inter{x}^{(0)}_i \leftarrow (\pi^{(0)}_i, \mu_i^{(0)}) \times \Inter{x}^*_i$ and let $\ell \leftarrow 0$.
    \WHILE{$\Inter{x}_i^{(\ell)} \neq \Inter{x}^*_i$}
        \STATE Let $b$ be the highest index such that $\NInter{X}^{(\ell)}_i({F^*}_i^b) > \NInter{X}^*_i({F^*}_i^b)$.
        \STATE Let $a$ be the lowest index such that for all $j \in a \cdots b$,
            $\NInter{X}^{(\ell)}_i({F^*}_i^j) > \NInter{X}^*_i({F^*}_i^j)$.
        \IF{$b = |T_i|$}
            \STATE Let $(\pi'_i, \mu'_i) \leftarrow \LowerTypes(\Inter{x}^{(\ell)}_i, a)$.
        \ELSE
            \STATE Let $(\pi'_i, \mu'_i) \leftarrow \MixTypes(\Inter{x}^{(\ell)}_i, a, b)$.
        \ENDIF
        \STATE Pick the largest $\alpha \in [0,1]$ for which still
            $\alpha\cdot (\pi'_i, \mu'_i)\times \Inter{x}^{(\ell)}_i+ (1-\alpha)\cdot\Inter{x}^{(\ell)}_i \succeq \Inter{x}_i$.
        \STATE Let $\Inter{x}^{(\ell+1)}_i \leftarrow
            \alpha\cdot (\pi'_i, \mu'_i)\times \Inter{x}^{(\ell)}_i+ (1-\alpha)\cdot\Inter{x}^{(\ell)}_i$.
        \STATE Let $(\pi^{(\ell+1)}_i, \mu^{(\ell+1)}_i) \leftarrow
            \alpha\cdot (\pi'_i, \mu'_i) \times (\pi^{(\ell)}_i, \mu^{(\ell)}_i)+ (1-\alpha)\cdot(\pi^{(\ell)}_i, \mu^{(\ell)}_i)$.
        \STATE $\ell \leftarrow \ell+1$.
    \ENDWHILE
    \MyRETURN $(\pi^{(\ell)}_i, \mu_i^{(\ell)})$.
\end{algorithmic}
\caption{\textsc{Compute\DPST{}}$(\Inter{x}^*_i, \Inter{x}_i)$} \label{alg:smap_comp}
\end{algorithm}

The next theorem implies Theorem~\ref{thm:smap}.
\begin{theorem}
\label{thm:smap_comp}%
For any $\Inter{x}_i$ and $\Inter{x}^*_i$ such that $\Inter{x}_i \succeq \Inter{x}^*_i$, the algorithm \ref{alg:smap_comp}
returns a \DPST{} $(\pi_i, \mu_i)$ such that $\Inter{x}^*_i = (\pi_i, \mu_i) \times \Inter{x}_i$. The algorithm runs for at most
$|T_i|$ iterations and runs in $O(|T_i|^3)$ time. Note that the size of the input of the algorithm is $O(|T_i|)$.
\end{theorem}
\begin{proof}
Let $J^{(\ell)}_+= \{j \in [|T_i|] | \NInter{X}^{(\ell)}_i(F_i^j) > \NInter{X}^*_i(F_i^j) \}$, i.e., $J^{(\ell)}_+$ is the
indices of all the points at which $\NInter{X}^{(\ell)}_i$ is strictly more than $\NInter{X}^*_i$. By induction it is easy to see
that all of the following statements hold at every iteration $\ell$ of the algorithm \ref{alg:smap_comp}.
\begin{enumerate}
\item \label{item:stm1}%
$\Inter{x}^{(\ell)}_i = (\pi^{(\ell)}_i, \mu^{(\ell)}_i) \times \Inter{x}_i$.

\item \label{item:stm2}%
$\Inter{x}^*_i \preceq \Inter{x}^{(\ell)}_i \prec \Inter{x}^{(\ell-1)}_i$.

\item \label{item:stm3}%
$|J^{(\ell+1)}_+| < |J^{(\ell)}_+|$. This can be shown as follows. If $\NInter{X}^{(\ell)}_i(q) =\NInter{X}^*_i(q)$ for some $q
\in [0,1]$ at some iteration $\ell=\ell'$, then it will also hold for the same $q$ and all iterations $\ell \ge \ell'$, so
$J^{(\ell+1)}_+ \subseteq J^{(\ell)}_+$. Furthermore, the way the algorithm chooses $\alpha$ at iteration $\ell$ implies that for
some index in $j \in a \cdots b$, $\NInter{X}^{(\ell)}_i(F_i^j) > \NInter{X}^*_i(F_i^j)$, but $\NInter{X}^{(\ell)+1}_i(F_i^j) =
\NInter{X}^*_i(F_i^j)$ which means $j \in J^{(\ell)}_+$ but $j \not \in J^{(\ell+1)}_+$ which proves the statement.
\end{enumerate}
Note that if $J^{(\ell)}_+ = \emptyset$, the second statement implies that $\Inter{x}^{(\ell)}_i=\Inter{x}^*_i$. But then the
last statement implies that the algorithm must stop after at most $|T_i|$ iterations. Finally, when the algorithm stops, the
first statement implies that $\Inter{x}^*_i = \Inter{x}^{(\ell)}_i = (\pi_i, \mu_i) \times \Inter{x}_i$. That completes the
proof.
\end{proof}

This completes the proof of Thoerem~\ref{thm:majorize}.
\end{proof}

\Xcomment{
\begin{proof}[Proof of Theorem~\ref{thm:smap_sym}]
 Note that \eqref{eq:MRM_k_sm} is a special case of \eqref{eq:MRM'_k} so it is necessary. We will show that it is also sufficient.
 We prove the theorem by explicitly constructing a symmetric ex-post allocation rule $x^*$ such that the corresponding interim
 allocation rules $\Inter{x}^*_i$ dominate $\Inter{x}_i$. By \autoref{thm:smap_comp}, a \DPST{} $(\pi_i, \mu_i)$ can be computed
 to convert $\Inter{x}^*_i$ to the the desired interim allocation $\Inter{x}_i$ and because of symmetry the same \DPST{} should
 work for all agents. Let $T_i = \{\Tp_i^1, \Tp_i^2, \cdots\}$ denote a relabeling of types in decreasing order of $\Inter{x}_i$
 and let $F_i^j = \sum_{r=1}^{j} f_i(\Tp_i^r)$. Suppose the vector of types reported by the agents is $t = (\Tp_1^{j_1},\cdots,
 \Tp_n^{j_n})$, so that $j_1, \cdots, j_n$ are the indices of the types reported by the agents. Define $x^*$ to be the following
 allocation rule. Choose the $k$ agents who have the lowest indices as the winners, breaking ties uniformly at random. To complete
 the proof, we need to show that the resulting interim allocations $\Inter{x}^*_i$ dominate the $\Inter{x}_i$. Let
 $\NInter{X}^*_i$ denote the resulting cumulative normalized interim allocation rule. For any $\bar{j} \in [|T_i|]$,
 $\NInter{X}^*_i(F_i^{\bar{j}})$ is the expected probability that agent $i$ has a type with index at most ${\bar{j}}$ and also
 wins, so $n\cdot\NInter{X}^*_i(F_i^{\bar{j}})$ is the expected number of winners whose type indices are at most ${\bar{j}}$,
 which is equal to the expected number of agents, up to $k$, whose types have index at most ${\bar{j}}$, i.e.,
 \begin{align*}
     n\cdot\NInter{X}^*_i(F_i^{\bar{j}}) &= \E_{j_1,\cdots,j_n}[\min(k, |\{i | j_i \le {\bar{j}}\}|)] \\
                                         &= g_k(F_i^{\bar{j}},\cdots, F_i^{\bar{j}})
 \intertext{on the other hand from \eqref{eq:MRM_k_sm} we can argue that}
     n\cdot\NInter{X}_i(F_i^{\bar{j}})   &\le g_k(F_i^{\bar{j}},\cdots, F_i^{\bar{j}})
 \end{align*}
 So $\NInter{X}_i(q) \le \NInter{X}^*_i(q)$ for all $q \in \{F_i^{\bar{j}} | \bar{j} \in [|T_i|]\}$. Since $\NInter{X}^*_i$ is
 concave and $\NInter{X}_i$ is piece-wise linear and its derivative changes only at $q \in \{F_i^{\bar{j}} | \bar{j} \in
 [|T_i|]\}$, it must be that $\NInter{X}_i(q) \le \NInter{X}^*_i(q)$ for all $q\in [0,1]$. That means $\Inter{x}^*_i$ dominates
 $\Inter{x}_i$, which completes the proof.
\end{proof}
}


==> conclusion.tex <==
\section{Extensions}
\label{sec:conclusion}

The paper has focused on continuous type spaces.  In \autoref{sec:nonmonotone} the algorithmic part requires discretization of the quantile spaces.  In \autoref{sec:ptas} we show that if the type space is continuous or large, we can get a PTAS by breaking the type space into $O(\log n / \epsilon)$ pieces.

In \autoref{sec:qapx}, we show that for unit-demand bidders whose valuations for different items are independent, there is a series of pricing schemes which sell with probability~$\quant$ that approximate~$\rev(\quant)$ within a constant factor, for each~$\quant$, and the set of agents served by these pricing schemes satisfies containment relationship as $\quant$ grows.  Therefore, the context free marginal revenue maximization procedure can be run (instead of the sampling procedures in \autoref{sec:monotone} and \autoref{sec:nonmonotone}) to achieve approximately optimal revenue.


==> hartline-notation.tex <==




\newcommand{\dd}[1]{\tfrac{\dd}{d#1}}

% accents for using with newagentvar
% (must take a single argument)
\newcommand{\ironed}{\bar}
\newcommand{\constrained}{\hat}
\newcommand{\optconstrained}{\composed{\optimized}{\constrained}}
\newcommand{\optimized}{\starred}
\newcommand{\differentiated}[1]{#1'}
\newcommand{\fortype}{\tilde}
 

\newcommand{\starred}[1]{#1^\star}
\newcommand{\noaccents}[1]{#1}
% compose accents on the fly
\newcommand{\composed}[3]{#1{#2{#3}}}



\newcommand{\newagentvar}[3][\noaccents]{%
\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{#3}}%
\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2smi\endcsname}[1][i]{#1{\boldsymbol{#3}}_{-##1}}%
\expandafter\newcommand\expandafter{\csname #2i\endcsname}[1][i]{#1{#3}_{##1}}%
\expandafter\newcommand\expandafter{\csname #2ith\endcsname}[1][i]{#1{#3}_{(##1)}}%
}

\newcommand{\newitemvar}[3][\noaccents]{%
\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{#3}}%
\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2smj\endcsname}[1][j]{#1{\boldsymbol{#3}}_{-##1}}%
\expandafter\newcommand\expandafter{\csname #2j\endcsname}[1][j]{#1{#3}_{##1}}%
\expandafter\newcommand\expandafter{\csname #2jth\endcsname}[1][j]{#1{#3}_{(##1)}}%
}





%
% perhaps don't use this.
%
\newagentvar{alloc}{x}


%
% in quantile space.
%
\newagentvar{quant}{q}
\newagentvar[\constrained]{exquant}{\quant}
\newagentvar[\constrained]{critquant}{\quant}  %remove?
\newagentvar[\optconstrained]{monoq}{\quant}

% remove these?
\newcommand{\quantp}{\exquant}
\newagentvar{qprice}{\price}
\newagentvar{qrev}{R}
\newagentvar[\ironed]{iqrev}{\qrev}





\newagentvar{qalloc}{y}
\newagentvar{cumalloc}{Y}
\newagentvar[\constrained]{calloc}{\qalloc}
\newagentvar[\constrained]{cumcalloc}{\cumalloc}
\newagentvar[\ironed]{ialloc}{\qalloc}
\newagentvar[\ironed]{icumalloc}{\cumalloc}

\newagentvar{rev}{R}
\newagentvar[\differentiated]{marg}{\rev}
\newagentvar{rawrev}{P}
\newagentvar[\differentiated]{rawmarg}{\rawrev}

\newagentvar[\tilde]{pseudorev}{\rev}
\newagentvar[\tilde]{pseudorawrev}{\rawrev}


%
% in value/type space
%

\newagentvar{typespace}{T}
\newagentvar{typesubspace}{S}

\newagentvar{type}{t}
\newagentvar{val}{v}

\newagentvar{price}{p}
\newagentvar{talloc}{\alloc}

\newagentvar[\constrained]{critval}{\val}
\newagentvar[\constrained]{reserve}{\val} % should this be used???
\newagentvar[\optconstrained]{monop}{v}


\newagentvar{util}{u}

% why two?
\newagentvar{strat}{s}
\newagentvar{bid}{b}



\newagentvar{virt}{\phi}
\newagentvar{qvirt}{\phi}
\newagentvar[\ironed]{ivirt}{\virt}


\newagentvar{dist}{F}
\newagentvar{dens}{f}
\newagentvar{hazard}{h}



\newagentvar[\ironed]{iprice}{\price}  %% what for?
\newagentvar[\ironed]{ival}{\val}  %% what for?

\newagentvar{ints}{{\cal I}}




\newcommand{\feasibles}{{\cal X}}




%
% for items
%

\newitemvar{pos}{j}
\newitemvar{weight}{w}
\newitemvar{udtype}{\type}
\newitemvar[\constrained]{udcrittype}{\type}
\newitemvar{udalloc}{\alloc}
\newitemvar{udprice}{\price}
\newitemvar[\constrained]{udcalloc}{\qalloc}
\newitemvar[\constrained]{udcumcalloc}{\cumalloc}






\newagentvar{mech}{{\cal M}}
\newagentvar{alg}{{\cal A}}



\newcommand{\dquant}{r}
\newcommand{\dval}{z}

\newcommand{\Rev}[1]{\mathbf{Rev}[#1]}
\newcommand{\MargRev}[1]{\mathbf{MargRev}[#1]}

\newcommand{\agind}[1][i]{_{#1}}


\newcommand{\indep}{{\cal I}}





\newcommand{\udmaxj}{\optimized{j}}
\newcommand{\udtypemax}{\udtypej[\optimized{j}]}


\newcommand{\udtypemin}{\type^{\min}}
\newcommand{\maxtype}{\type^{\max}}
\newcommand{\lagrange}{\lambda}
\newcommand{\budget}{B}




\newcommand{\iG}{\bar{G}}
\newcommand{\ig}{\bar{g}}
\newcommand{\iq}{\bar{q}}

\newcommand{\game}{G}





\newcommand{\rawprice}{\price^{\game}}
\newcommand{\rawprices}{\prices^{\game}}
\newcommand{\rawpricesmi}{\rawprices_{-i}}
\newcommand{\rawpricei}[1][i]{\rawprice\agind[#1]}




\newcommand{\rawalloc}{\alloc^{\game}}
\newcommand{\rawallocs}{\allocs^{\game}}
\newcommand{\rawallocsmi}{\rawallocs_{-i}}
\newcommand{\rawalloci}[1][i]{\rawalloc\agind[#1]}



\newcommand{\zeros}{{\mathbf 0}}
\newcommand{\ones}{{\mathbf 1}}



\newcommand{\cost}{c}

\DeclareMathOperator{\OPT}{OPT}
\DeclareMathOperator{\Vic}{Vic}
\DeclareMathOperator{\Mye}{Mye}
\DeclareMathOperator{\VCG}{VCG}
\DeclareMathOperator{\SM}{SM}
\DeclareMathOperator{\RM}{RM}
\DeclareMathOperator{\VSM}{VSM}
\DeclareMathOperator{\IVSM}{IVSM}

\DeclareMathOperator{\EF}{EF}
\DeclareMathOperator{\EFO}{EFO}
\DeclareMathOperator{\RSEM}{RSEM}
\DeclareMathOperator{\RSOP}{RSOP}
\DeclareMathOperator{\RSPE}{RSPE}

\DeclareMathOperator{\surplus}{Surplus}
\DeclareMathOperator{\IID}{IID}
\DeclareMathOperator{\profit}{Profit}

\DeclareMathOperator{\REF}{REF}
\DeclareMathOperator{\APX}{APX}

\def\BM{\REF}
\def\PERF{\APX}


\newcommand{\poly}{{\cal P}}
\newcommand{\Lot}{{\cal L}}
\newcommand{\np}{{\cal NP}}
\newcommand{\algo}{{\cal A}}
\newcommand{\auction}{{\cal A}}
\newcommand{\mecha}{{\cal M}}
\newcommand{\ialgo}{\bar{\cal A}}

\newcommand{\osp}{{\cal F}}
\newcommand{\osps}{\osp \super 2}

\newcommand{\EFOs}{\EFO \super 2}
 
\newcommand{\bm}{{\cal G}}
\newcommand{\bms}{\bm \super 2}

%\newcommand{\setsize}[1]{{\left|#1\right|}}

\newcommand{\reals}{{\mathbb R}}
\newcommand{\posreals}{\reals_+}






\newcommand{\thealloc}{\hat{\alloc}}
\newcommand{\analloc}{\alloc\primed}


\newagentvar{trans}{\sigma}

\newagentvar{demandset}{S}

\newcommand{\primed}{^\dagger}
\newcommand{\doubleprimed}{^{\ddagger}}
\newcommand{\pprimed}{\doubleprimed}

\newagentvar{distout}{w}
\newagentvar{idistout}{\bar{w}}

\newcommand{\rsmsize}{m}

\newcommand{\metric}{c}


\newcommand{\implements}{\preceq}
\newcommand{\isimplementedby}{\succeq}


%
% matroid definitions.
%
\DeclareMathOperator{\matrank}{rank}
\newcommand{\rank}{\matrank}            % xphase this out.
\newcommand{\matset}{S}
\newcommand{\matground}{N}
\newcommand{\matindeps}{{\cal I}}


%% correlation gap, set functions

\newcommand{\cset}{S}
\newcommand{\setfunc}{g}
\newcommand{\setdist}{{\cal D}}
\newcommand{\margsetdist}{\setdist^{I}}


%% prophet inequality
\newcommand{\gamblerpayoff}{G}
\newcommand{\prophetpayoff}{P}
\newcommand{\prnosale}{\chi}
\newcommand{\Ei}{{\cal E}_i}

\newcommand{\numpieces}{Q}

\newcommand{\rejectset}{\perp}


\newcommand{\threshutil}{\mu}

\newcommand{\convexcomb}{\alpha}


\newcommand{\concavefunc}{h}


==> lin-ord-app.tex <==
\section{Proofs from \autoref{sec:general}}
\label{sec:lin-ord-app}

In this appendix we prove \autoref{greedylemma} and \autoref{l:nested}.

\noindent{\bf \autoref{greedylemma} (Restatement).}
For a revenue-linear single-agent problem, let $\qalloc$ be the
optimal allocation rule subject to some constraint $\calloc$. Then,
for any $\exquant$ such that $\rev''(\exquant)\neq 0$ we have
$\cumalloc(\exquant) = \cumcalloc(\exquant).$

\begin{proof}
Since $\qalloc$ is the optimal allocation rule subject to $\calloc$, we have
$\Rev{\qalloc} = \Rev{\calloc}$.
Linearity implies that
\begin{equation*}
\MargRev{\calloc} = \int_{0}^1 \qalloc(\quant)\rev'(\quant)\, \dd\quant = \int_{0}^1
\calloc(\quant)\rev'(\quant)\, \dd\quant = \MargRev{\qalloc}.
\end{equation*}

Integrating by parts, we have
\begin{equation}
\inteval{\cumalloc(\quant)\rev'(\quant)}_{0}^1 - \int_{0}^1
\cumalloc(\quant)\rev''(\quant)\,\dd\quant =
\inteval{\cumcalloc(\quant)\rev'(\quant)}_{0}^1- \int_{0}^1
\cumcalloc(\quant)\rev''(\quant)\,\dd\quant.
\label{firsteqingreedy}\end{equation}


Note that $\calloc$ and $\qalloc$ have the same ex ante probability of allocation $\cumcalloc(1) = \cumalloc(1)$;
also by definition $\cumalloc(0) = \cumcalloc(0) = 0$.  Combining these observations with
\eqref{firsteqingreedy} we have
\begin{equation*}
\int_{0}^1 \cumalloc(\quant)\rev''(\quant)\,\dd\quant = \int_{0}^1
\cumcalloc(\quant)\rev''(\quant)\,\dd\quant,
\end{equation*}
and therefore,
\begin{equation}
\int_{0}^1 [\cumalloc(\quant)-\cumcalloc(\quant)]\rev''(\quant)\,\dd\quant = 0. \label{secondeqingreedy}
\end{equation}

Notice that for any $\quant$, $\cumalloc(\quant) - \cumcalloc(\quant)$ and $\rev''(\quant)$ are non-positive
(by domination and concavity, respectively) so their product is non-negative.  Therefore,
\eqref{secondeqingreedy} can be satisfied only if $[\cumalloc(\quant)-\cumcalloc(\quant)]\rev''(\quant)= 0$
for all $\quant$. This implies that if $\rev''(\quant)<0$, then we must have $\cumalloc(\quant) =
\cumcalloc(\quant)$, which completes the proof.
\end{proof}

Recall that for any $\exquant$ where $\rev''(\exquant) \neq 0$, we defined $\typespace_{\exquant}$ to be
the set of types allocated (with full lotteries) in the optimal lottery pricing
subject to $\callocstep$. 

\noindent {\bf \autoref{l:nested} (Restatement)}
For a revenue-linear single-agent problem, for any $\exquant_1>\exquant_2$ and
$\rev''(\exquant_1),\rev''(\exquant_2)\neq 0$, we must have
$\typespace_{\exquant_1} \supseteq \typespace_{\exquant_2}$.

% \begin{lemma}
% For a revenue-linear single-agent problem, for any $\quant_1>\quant_2$ and
% $\rev''(\quant_1),\rev''(\quant_2)\neq 0$, we must have $\typespace_{\quant_1} \supseteq
% \typespace_{\quant_2}$.
% \end{lemma}

\begin{proof}
Assume for contradiction that $\typespace_{\exquant_2}\backslash \typespace_{\exquant_1} \neq \emptyset$. Let
$\alpha = \dist(\typespace_{\exquant_2}\backslash \typespace_{\exquant_1})>0$. Consider the following allocation
constraint
\begin{align*}
    \calloc(\quant) &=
        \begin{cases}
            1 & \quant\leq \exquant_2 \\
            1/2 & \exquant_2 < \quant \leq \exquant_1 \\
            0 & \exquant_1 < \quant.
        \end{cases}
\end{align*}
By revenue linearity, the revenue of the optimal auction subject to $\calloc$ is
$[\rev(\exquant_1)+\rev(\exquant_2)]/2$. Notice that the mechanism that runs
$\rev(\exquant_1)$ and $\rev(\exquant_2)$ each with probability 1/2 achieves this revenue. The allocation rule $\qalloc$ of this
mechanism is
\begin{align*}
    \qalloc(\quant) &=
        \begin{cases}
            1 & \quant\leq \quant_2-\alpha \\
            1/2 & \quant_2-\alpha \leq \quant \leq \quant_1 + \alpha \\
            0 & \quant_1 + \alpha \leq \quant.
        \end{cases}
\end{align*}
Notice that this allocation rule is dominated by $\calloc$, and achieves the optimal revenue. Yet, we have
\begin{align*}
\cumcalloc(\exquant_1) = \int_{\quant = 0}^{\exquant_1} \calloc(\quant)\:\dd\quant > \int_{\quant=0}^{\exquant_1} \qalloc(\quant)\:\dd\quant = \cumalloc(\exquant_1).
\end{align*}
This contradicts \autoref{greedylemma}.
\end{proof}

%\paragraph{Downward-close environments}
%
%The preceding construction applies generally for any feasibility
%constraint.  If we restrict attention to downward-closed feasibility
%constraints then


==> linearity.tex <==
\STOC{
\section{Proof that revenue-linearity implies orderability}
\label{sec:linearity}
}


\IFSTOCELSE{We motivate and prove \autoref{thm:linear=orderable}.
%%This proof sheds insight on Myerson's ironing proceedure.

}
{In the remainder of this section we give a proof of
\autoref{thm:linear=orderable}, i.e., that revenue linearity implies
orderability.}
By the definition of marginal revenue maximization an agent is
(potentially) treated distinctly with quantiles with different
marginal revenue and identically for quantiles with the same marginal
revenue.  It is also obvious for quantiles in intervals where the
revenue is locally linear (therefore: the marginal revenue is constant
and the second derivative of the revenue curve is zero) can never be
the critical quantiles in Step~\ref{step:critical-quantiles} of the
marginal revenue mechanism and therefore the corresponding step
mechanisms are never used.  These structural properties are not that
useful, however, if there is not a fixed mapping from type space to
quantile space.  Indeed, the main challenge of multi-dimensional
mechanism design is that there is no explicit ordering on type space;
revenue linearity, however, implies that there is an implicit fixed
mapping.  Consequently, much of the intuition for optimal mechanisms
for single-dimensional agents extends to optimal mechanisms for
context-free agents.

The intuition behind this proof comes from connecting our marginal
revenue approach to Myerson's theory of ironing for single-dimensional
agents.  For single dimensional types there is a natural ordering on
types and a revenue curve can be defined by considering mechanisms
that serve the top $\quant$ quantile of types by this ordering.  In
these step mechanisms a type is either served or not served with
probability one.  This revenue curve may not be concave and must
therefore be ironed (by mixing between deterministic step mechanisms)
to get a concave revenue curve.  The step mechanism that correspondes
to mixing between two step mechanisms does not serve agents with
probability one.  Instead it has three levels: high types are served
with probability one, medium types are served with the same constant
probability (depending on the probabilities of the convex
combination), and low times are served with probability zero.
However, again because the revenue curve is linear (second derivative
of the revenue $\rev''(\quant)$ is zero) on such an interval these
mixed step mechanisms are never used.  This exact same structure
generalizes to context-free agents.


\begin{lemma}
\label{lem:opt-saturate}
For a revenue-linear single-agent problem, let $\qalloc$ be the optimal allocation rule subject to some constraint $\calloc$. Then, for any $\quant$ such that $\rev''(\quant)\neq 0$ we have $\cumalloc(\quant) = \cumcalloc(\quant)$.
\label{greedylemma}\end{lemma}
\begin{proof}
Since $\qalloc$ is the optimal allocation rule subject to $\calloc$, then we
have, by definition, $\Rev{\qalloc} = \Rev{\calloc}$. Linearity implies that\IFSTOCELSE{}{ (working from inside out)}:
\IFSTOCELSE
{\begin{align*}
\Rev{\qalloc} &= \Rev{\calloc}\\
\MargRev{\qalloc}&=\MargRev{\calloc}\\
\int_{0}^1 \qalloc(\quant)\rev'(\quant)\:\dd\quant &=  \int_{0}^1 \calloc(\quant)\rev'(\quant)\:\dd\quant.
\end{align*}
}
{\begin{equation*}
\int_{0}^1 \qalloc(\quant)\rev'(\quant)\:\dd\quant = \MargRev{\qalloc} =
\Rev{\qalloc} = \Rev{\calloc} = \MargRev{\calloc} = \int_{0}^1 \calloc(\quant)\rev'(\quant)\:\dd\quant.
\end{equation*}}

Integrating by parts, we have
\begin{align}
\STOC{\notag&}\inteval{\cumalloc(\quant)\rev'(\quant)}_{0}^1 - \int_{0}^1
\cumalloc(\quant)\rev''(\quant)\,\dd\quant \STOC{\\&\qquad}=
\inteval{\cumcalloc(\quant)\rev'(\quant)}_{0}^1- \int_{0}^1
\cumcalloc(\quant)\rev''(\quant)\,\dd\quant.
\label{firsteqingreedy}\end{align}


By definition, $\calloc$ and $\qalloc$ have the same ex ante probability of
allocation, $\cumcalloc(1) = \cumalloc(1)$; by definition $\cumalloc(0)
= \cumcalloc(0) = 0$.  Substituting these into~\eqref{firsteqingreedy}, we have
\begin{equation*}
\int_{0}^1 \cumalloc(\quant)\rev''(\quant)\,\dd\quant = \int_{0}^1 \cumcalloc(\quant)\rev''(\quant)\,\dd\quant,
\end{equation*}
or 
\begin{equation}
\int_{0}^1 [\cumalloc(\quant)-\cumcalloc(\quant)]\rev''(\quant)\,\dd\quant = 0.
\label{secondeqingreedy}
\end{equation}

Notice that for any $\quant$, $\cumalloc(\quant) - \cumcalloc(\quant)$
and $\rev''(\quant)$ are non-positive (by domination and concavity,
respectively) so their product is non-negative.  Therefore,
\eqref{secondeqingreedy} can be satisfied only if
$[\cumalloc(\quant)-\cumcalloc(\quant)]\rev''(\quant)= 0$ for all
$\quant$. This implies that if $\rev''(\quant)<0$, then we must have
$\cumalloc(\quant) = \cumcalloc(\quant)$, which completes the proof.
\end{proof}

\autoref{lem:opt-saturate} in particular implies that for $\quant$
with $\rev''(\quant) \neq 0$ the $\quant$-step mechanism (for step
constraint $\callocstep$) has allocation rule $\qallocstepopt =
\callocstep$.  I.e., the $\quant$-step mechanism has full lotteries
only (i.e., each type either is served with probability 1 or 0).


For any such $\quant$, define $\typespace_{\quant}$ to be the set of
types allocated (with full lotteries) in the optimal allocation
subject to $\callocstep$. The following lemma shows that these sets are
nested.

\begin{lemma}
For a revenue-linear single-agent problem, for any $\quant_1>\quant_2$ and
$\rev''(\quant_1),\rev''(\quant_2)\neq 0$, we must have
$\typespace_{\quant_1} \supseteq \typespace_{\quant_2}$.
\end{lemma} 

\begin{proof}
Assume for contradiction that
$\typespace_{\quant_2}\backslash \typespace_{\quant_1} \neq
\emptyset$. Let $\alpha =
\dist(\typespace_{\quant_2}\backslash \typespace_{\quant_1})>0$. Consider
the following allocation constraint:
\begin{align*}
    \calloc(\quant) &=
        \begin{cases}
            1 & \quant\leq \quant_2 \\
            1/2 & \quant_1 \leq \quant \leq \quant_2 \\
            0 & \quant_1 \leq \quant.
        \end{cases}
%\end{align*}
\intertext{By revenue linearity, the revenue of the optimal auction subject to
$\calloc$ is $[\rev(\quant_1)+\rev(\quant_2)]/2$. Notice that the
mechanism that runs $\rev(\quant_1)$ and $\rev(\quant_2)$ each with
probability 1/2 achieves this revenue. The allocation rule $\qalloc$
of this mechanism is:}
%\begin{align*}
    \qalloc(\quant) &=
        \begin{cases}
            1 & \quant\leq \quant_2-\alpha \\
            1/2 & \quant_2-\alpha \leq \quant \leq \quant_1 + \alpha \\
            0 & \quant_1 + \alpha \leq \quant.
        \end{cases}
\end{align*}
Notice that this allocation rule is dominated by $\calloc$, and achieves the optimal revenue. Yet, we have
\begin{align*}
\cumcalloc(\quant_1) = \int_{\quant = 0}^{\quant_1} \calloc(\quant)d\quant > \int_{\quant=0}^{\quant_1} \qalloc(\quant)d\quant = \cumalloc(\quant_1).
\end{align*}
This contradicts~\autoref{greedylemma}.
\end{proof}

%\paragraph{Downward-close environments}
%
%The preceding construction applies generally for any feasibility
%constraint.  If we restrict attention to downward-closed feasibility
%constraints then 


==> marg.tex <==
\section{(Generalized) Marginal Revenue Maximization}
\label{sec:marg}





\paragraph{A Heuristic Generalization To Service Constrained Environments}


==> monotone-app.tex <==
\section{Proof from \autoref{sec:monotone}}
\label{sec:monotone-app}

\begin{proof} [Proof of \autoref{claim:monallocq-ex}]
Monotonicity is obvious.  We only need to show that the expectation of $\allocq{i}{\quant}{\type_i}$
is~$\quant$. When $\quant < \thresholdq_i$, this is true by definition of~$\mecq{i}{\quant}$; and when $\quant >
\thresholdq_i$, $\monallocq{i}{\quant}{\type_i}$ is simply a linear interpolation between
$\allocq{i}{\thresholdq_i}{\type_i}$ and~$1$, and therefore its expectation over types is also linear on
$[\thresholdq_i, 1]$.  Given that $\Ex[\type_i]{\allocq{i}{\thresholdq_i}{\type_i}} = \thresholdq_i$, we know that the
claim is also true on $[\thresholdq_i, 1]$.
\end{proof}


In the proof of \autoref{thm:monotone-sample} we assume that $\monallocq{i}{\quant}{\type_i}$ is continuous in~$\quant$ for
all~$\type_i$, i.e., $\allocq{i}{\quant}{\type_i}$ is continuous for $\quant \in [0, \thresholdq_i]$.  This is just to guarantee that $\quant_i$ sampled in \autoref{proc:monotone-sample} does not lump in
a point mass, which simplifies the proof for feasibility (\autoref{lem:monotone-feasible}).  This assumption can be
easily removed by adding a tie-breaking rule in \autoref{proc:monotone-sample} and \autoref{proc:maxRprime}.


\begin{proof}[Proof of \autoref{lem:monotone-uniformq}]
It suffices to show that the distribution has the correct cummulative density function, i.e.,
$\Ex[\type_i]{\Prx[\quant_i]{\quant_i \leq q}} = \quant$ for any $\quant \in [0, 1]$.  By definition, this is
$\Ex[\type_i]{\monallocq{i}{\quant}{\type_i}}$, which is $\quant$ by \autoref{claim:monallocq-ex}.
\end{proof}


\begin{proof}[Proof of \autoref{lem:monotone-probq}]
We first justify that when $\quant_{-i}$ determines a $\thrcontextq_i$ for agent~$i$, we are effectively running
$\mecq{i}{\thrcontextq_i}$ for agent~$i$.  When this happens, with probability $\Prx[\quant_i]{\quant_i \leq \thrcontextq_i}$ we
run the outcome rule of~$\mecq{i}{\thrcontextq_i}$ conditioning on that we serve~$\type_i$.  But $\Prx[\quant_i]{\quant_i
\leq \thrcontextq_i}$ is exactly $\monallocq{i}{\thrcontextq_i}{\type_i}$, which is equal to $\allocq{i}{\thrcontextq_i}{\type_i}$
(since $\thrcontextq_i \leq \thresholdq_i$), the probability with which $\mecq{i}{\thrcontextq_i}$ would
serve~$\type_i$ in the first place.  The same argument goes for the case when we do not serve~$\type_i$.  Hence in
effect we are simply running $\mecq{i}{\thrcontextq_i}$.

With this shown, comparing \autoref{proc:monotone-sample} and \autoref{proc:maxRprime}, we see that the only remaining
difference is that in \autoref{proc:maxRprime}, the $\quant_{-i}$ used to determine $\thrcontextq_i$
are drawn uniformly independently from~$[0, 1]$, whereas in \autoref{proc:monotone-sample} these quantiles are from a
sampling process that depends on the other agents' types.  But as \autoref{lem:monotone-uniformq} shows, the two
distributions are the same, and hence the two procedures arrive at exactly the same distribution over
$\mecq{i}{\quant}$'s for each agent~$i$.
\end{proof}



\begin{proof}[Proof of \autoref{lem:monotone-feasible}]
Recall that we serve an agent only when $\quant_i \leq \thrcontextq_i$.  Since $\monallocq{i}{\quant}{\type_i}$ is continuous
in~$\quant$, the probability that $\quant_i$ is equal to $\thrcontextq_i$ is~$0$.  Therefore, with probability~$1$,
$\quant_i \neq \thrcontextq_i$ for all~$i$.  Then serving an agent means $\marrevq{i}{\quant_i} < \marrevq{j}{\quant_j}$ for
all $j \neq i$.  This can happen to at most one~$i$, hence the mechanism is feasible.
\end{proof}


\begin{proof}[Proof of \autoref{lem:monotone-truthful}]
As shown in \autoref{lem:monotone-uniformq}, once $\thrcontextq_i$ is determined, we are running $\mecq{i}{\thrcontextq_i}$ for
agent~$i$, which is truthful by definition.  In addition, $\thrcontextq_i$ is determined solely by the independent random
variables $\quant_{-i}$ and the function $\marrevq{i}{\quant}$, both of which cannot be affected by the agent's bid.  So
the mechanism is simply a distribution over truthful mechanism, and is also truthful.
\end{proof}


%\begin{proof}[Proof of \autoref{thm:monotone-sample}]
%\end{proof}


==> qapx.tex <==
\newcommand{\auc}{A^p}
\newcommand{\aucl}{A^l}
\newcommand{\price}{p}
\newcommand{\mecqp}{M^p}
\section{Simple approximations for $\rev(\quant)$}
\label{sec:qapx}

In this section, we generalize the results in \cite{CHK07} and
\cite{CMS-10} for general $\quant$.
\begin{definition}
For a given instance of unit demand, single agent with $m$ items,
\emph{$m-$copy} representation is defined by making $m$ clones of
the agent and one item. The valuation of clone $j$ for the single
item is the same as the valuations of the single agent for item $j$
in original representation.
\end{definition}
We will abuse the notation and refer to the single agent with $m$
items, single agent representation. We show that item pricing is a
$2$-approximation of general $\mecq{i}{q}$. Next, we show that the
expected revenue from item pricing for single agent representation
is at most as much as the revenue of \emph{$m-$copy} representation.
And finally we show that offering uniform ironed virtual price to
all agents obtains a $2$-approximation for $m-$copy representation.
Reversing the process yields a $4$-approximation algorithm for
$\rev(q)$ by offering one uniform virtual price.

\begin{lemma}
For a given $\quant$ and any product distribution $\Dist = \Dist_1
\times \ldots\times \Dist_m$, the expected revenue of optimal
single-agent, $m$-item pricing (call the mechanism $\mecqp(\quant)$
and the expected revenue of such mechanism $\Rev{\mecqp(\quant)}$ is
at most the revenue of $m$-copy representation with the expected
probability of allocation $\quant$.
\end{lemma}
\begin{proof}
Similar to \cite{CHK07}, using $\mecqp(\quant)$, we construct an
auction $\auc(\quant)$ for $m$-copy representation and we show that
the expected revenue of such mechanism is at least
$\Rev{\mecqp(\quant)}$. Define $i^* = \argmax_i (v_i - \price_i)$.
In the $m$-copy representation, $\auc(q)$ allocates to $i^{*}$ and
will charge $i^*$ $\tau\ge \price_{i^{*}}$ which is the critical
threshold of payment for $i^*$ to stay winner. It is clear that
$\auc(\quant)$ is truthful. Also note that the probability of
allocation in $\auc(\quant)$ is at most $\quant$. The item will be
allocated in $\auc(\quant)$ iff  $ \exists j: \ v_j - p_j>0$.
Similarly in single agent representation, $\mecqp(\quant)$ will
allocate to the single agent one of the items iff at $\exists j \
v_j - p_j\ge 0$. Assuming that $\mecqp(q)$ allocates with
probability at most $q$ to the single agent, we guarantee that the
expected probability of allocation in $\auc$ is also at most $q$.
Finally, note that there is a one to one mapping between the
allocation in $\mecqp(q)$ and $\auc$. However in every mapping the
payment in $\auc(\quant)$ is at least as high as $\mecqp(q)$ which
completes the proof.
\end{proof}
\begin{lemma}
\label{lemma:copy}
For any independent, unit demand, single agent
environment with probability of allocation at most $\quant$ in
expectation, a uniform ironed virtual price is a $2$-approximation
to the optimal price revenue with expected probability of allocation
at most $\quant$.
\end{lemma}
\begin{proof}
First, note that to design a mechanism for independent, unit demand
single agent environment, it is sufficient to design a sequential
posted pricing mechanism with uniform constant ironed virtual value,
since in the sequential posted pricing we consider the worst
possible ordering. The proof is based on the generalization of
prophet inequality for general $\quant$. We prove that there exists
a threshold $t$ for which the expected revenue of the gambler is at
least half of the expected value of the maximum prize. We first
compute an upperbound for the optimal revenue and then a lowerbound
for the obtained revenue by the uniform virtual price. Since the
probability of allocation is upperbounded by $q$, the upperbound is
defined by the expected value of the highest agent conditioned on
the fact that it is higher than some threshold. To get an upperbound
on this value we choose the threshold such that this event happens
with probability exactly equal to $q$. Let us call the threshold
$\tau$. Now the upperbound on the optimal revenue is defined by
\begin{align}
\label{eqn:opt}
OPT &\le q \cdot \tau + \max_i(0,v_i-\tau)\\
&\le q\cdot\tau+ \sum_{i}\Ex{v_i \in V}{(v_i-\tau)^+}
\end{align}
Now to compute a lowerbound of the extracted profit by the uniform
virtual price, we assume the worst arrival scenario. We set the
uniform virtual price equal to $\tau$. The lowerbound can be defined
by:
\begin{align}
\label{eqn:apx} APX &\ge \tau\cdot q + \sum_i \Ex[v_i\in V]{(v_i
-t)^+| \ \forall j \neq i\  v_j<
\tau}\cdot P(\forall j \ v_j < \tau)\\
&\ge \tau \cdot q + (1-q)\cdot \sum_i \Ex[v_i \in V]{(v_i-t)^+}\\
\end{align}
Now we consider $2$ cases:
\begin{itemize}
\item
if $\quant \ge \frac{1}{2}$, based on lemma[9] in \cite{CHK07}, we
already know that the uniform virtual price with
$\quant=\frac{1}{2}$ obtains at least half of the optimal with $q=1$
which itself is an upperbound for the optimal solution for smaller
$\quant$.
\item
Or $\quant \le \frac{1}{2}$. In this case we have $1-\quant \ge
\frac{1}{2}$. Comparing \autoref{eqn:opt}, \autoref{eqn:apx}, we can
see that the uniform virtual price obtains at least half of the
optimal (and in fact the ratio improves as $\quant$ gets smaller.
More accurately, the uniform ironed virtual price obtains
$\max(\frac{1}{2},1-\quant)$ of the optimal solution.
\end{itemize}
\end{proof}

\begin{lemma}
\label{lemma:lotteryq} For any product distribution $\Dist =
\Dist_1\times\ldots \times\Dist_m$ the expected revenue of optimal
single-agent lottery pricing with the expected probability of
allocation at most $\quant$ is at most twice of the optimal auction
with expected probability of allocation $\quant$ for $m-$copy
representation.
\end{lemma}
\begin{proof}
Similar to \autoref{lemma:copy}, we construct an auction $\aucl(q)$
for $m-$copy from the optimal lottery pricing and we show that it
obtains at least half of the revenue of the optimal lottery (denoted
by $OPT_l$). Consider a valuation $v$ and suppose the agent selects
lottery $l=((q_1,\ldots,q_m),p)$. The utility of this agent at the
lottery pricing is defined by $\sum_{i=1}^m v_i\cdot q_i -p$.
Without loss of generality suppose: $v_1 \ge v_2\ge \ldots\ge v_m$.
For $m-$copy representation, $\aucl(\quant)$ allocates the item to
the clone with value $v_1$ with probability $q_1$ and charge him
$p-\sum_{j\neq 1}v_j\cdot q_j$. It is clear that the utility of the
clone $1$ in $\aucl(\quant)$ is exactly equal to the utility of the
single agent in lottery pricing. Since $l$ was the utility
maximizing lottery for the single agent, our auction is also
incentive compatible. It is also clear that the expected probability
of allocation is at most $\quant$ in the new auction. Next, we show
how to bound the revenue of our auction. Let us define $Q(v) =
\sum_{i=1}^m q_i$.The revenue of our auction is :
\begin{align*}
\Rev{\aucl(q)}&= p - \sum_{j \neq 1}q_j\cdot v_j\\
&\ge p - Q(v) \cdot v_2\\
\end{align*}
Now, consider an auction that in our $m-$copy representation that
allocates to $v_1$ and charge him $v_2$ iff $v_2 \ge \tau$ and
select $\tau$ such that this event happens with probability exactly
$\quant$. It is clear that the expected probability of allocation is
at most $\quant$. Also the expected payment of this auction is at
least as much as  $\Ex[v\in V]{Q(v)\cdot v_2}$ subject to $\Ex[v\in
V]{Q(v)} \le q$. Also it is easy to argue that this auction is
incentive compatible. As a result, $OPT_l$ is at most twice
$\Rev{\aucl(\quant)}$.
\end{proof}
\begin{remark}
Conditioned on \autoref{cond:linear-rev}, if we have an $\alpha$
approximation to $\rev(\quant)$, we obtain an $\alpha$ approximation
to the optimal revenue.
\end{remark}


==> qapx2.tex <==
\newcommand{\auc}{A^p}
\newcommand{\aucl}{A^l}
\newcommand{\price}{p}
\newcommand{\mecqp}{M^p}
\newcommand{\thr}{t}

\paragraph{Unit-demand approximation.}
\label{sec:qapx} 


In this section, we present a simple approximate marginal revenue
mechanism and show that it is a $4-$approximation to the optimal
revenue for single agent, $m-$item with unit demand constraint subject
to any given interim allocation feasibility constraint. We assume that
the type of each agent is drawn from a product distribution
$F=F_1\times \cdot\times F_m$. \cite{CHK07} and \cite{CMS-10},
presented an approximation optimal pricing mechanism for the similar
setting without having the interim feasibility constraint. In this
section, we show that with the extra constraint $\qalloc_i(\cdot)$ on
the interim allocation feasibility , still we can obtain a simple
approximation mechanism to the optimal revenue $\Rev{\qalloc_i}$ for
single agent unit demand problem. In the rest of the section, we will
refer to our original problem with a single agent with $m$ items and
unit demand constraint, the \emph{original environment}.  As in
\cite{whatisthisreference}, we first present a single dimensional
setting (we will call it \emph{representative environment} in which
the optimal revenue is an upper bound for the optimal revenue of our
setting. We show that item pricing is a $2$-approximation of general
$\Rev{\qalloc_i}$. Next, we show that the expected revenue of optimal
item pricing for original environment is at most as much as the
optimal revenue of the representative environment. Representative
environment in short, is to replace an agent interested to $m-$ items
with $m$ clones of the agent and one item (we will describe
representative environment in more detail in \autoref{def:m-copy}).
And finally we show that offering the uniform ironed virtual price to
all agents obtains at least half of the optimal revenue of the
representative environment. Reversing the process yields a simple
$4$-approximation algorithm for $\rev(\qalloc(\cdot))$ by optimizing
over marginal-uniform-ironed-virtual-prices.
\begin{definition}[Representative environment]
\label{def:m-copy} For a given instance of unit demand, single agent
with $m$ items, \emph{representative environment} is defined by
making $m$ clones of the agent and one item. The valuation of clone
$j$ for the single item is the same as the valuations of the single
agent for item $j$ in the single agent environment.
\end{definition}


\begin{lemma}
For a given $\qalloc(\quant)$ and any product distribution $\Dist =
\Dist_1 \times \ldots\times \Dist_m$, let $p$ be an item pricing for
which some item is bought with probability $\qalloc(\quant)$ , then
there is an auction for the representative environment that serves
with probability $\qalloc(\quant)$ and its revenue is at least as
much as the revenue of pricing mechanism $p$ in \emph{single agent}
environment.
\end{lemma}
%should I drop the proof and just put a reference?
\begin{proof}
Similar to \cite{CHK07}, using $\mecqp(\quant)$, we construct an
auction $\auc(\quant)$ for $m$-copy representation and we show that
the expected revenue of such mechanism is at least
$\Rev{\mecqp(\quant)}$. Define $i^* = \argmax_i (v_i - \price_i)$.
In the $m$-copy representation, $\auc(q)$ allocates to $i^{*}$ and
will charge $i^*$ $\tau\ge \price_{i^{*}}$ which is the critical
threshold of payment for $i^*$ to stay winner. It is clear that
$\auc(\quant)$ is truthful. Also note that the probability of
allocation in $\auc(\quant)$ is at most $\quant$. The item will be
allocated in $\auc(\quant)$ iff  there exists $j$ for which $\ v_j -
p_j>0$. Similarly in the original environment, $\mecqp(\quant)$ will
allocate to the single agent one of the items if and only if there
exists $j$ for which $v_j - p_j\ge 0$. Assuming that
$\mecqp(\quant)$ allocates with probability at most $\quant$ to the
single agent, we guarantee that the expected probability of
allocation in $\auc$ is also at most $\quant$. Finally, note that
there is a one to one mapping between the allocation in
$\mecqp(\quant)$ and $\auc$. However in every mapping the payment in
$\auc(\quant)$ is at least as high as $\mecqp(\quant)$ which
completes the proof.
\end{proof}
Also the obtained revenue in original environment is at least as
much as the revenue of the sequential posted pricing in the
representative environment. So it is sufficient to present a
sequential posted pricing approximation mechanisms for
representative environments. In the next lemma, we first show that
for a given $\quant$, using sequential uniform ironed virtual price
achieves a $2-$ approximation to the optimal pricing mechanism.
\begin{lemma}
\label{lemma:copy} Given an instance of the representative
environment with type distribution of the clones coming from $F$ and
for a given interim feasibility constraint $\quant$, a sequential
posted pricing with uniform ironed virtual price is a
$2$-approximation to the optimal price revenue that satisfies
interim feasibility constraint $\quant$.
\end{lemma}
\begin{proof}
The proof is based on the generalization of prophet inequality for
general $\quant$. We prove that there exists a threshold $\tau$ for
which the expected revenue of the gambler is at least half of the
expected value of the maximum prize conditioned on interim
allocation $\quant$. We first compute an upper bound for the optimal
revenue of the representative environment conditioned on interim
allocation feasibility $\quant$. Since the probability of allocation
is at most $\quant$, the optimal solution is upper bounded by the
expected value of the highest clone conditioned on item being
allocated with probability at most $\quant$ which would be
translated to the value of the highest clone being higher than some
given threshold to satisfy the interim allocation feasibility
constraint. To maximize the upper bound, the threshold should be
chosen in a way that the highest clone would be greater than the
threshold with probability exactly equal to $\quant$. Let us call
the threshold $\tau$. The upper bound on the optimal revenue is:
\begin{align}
\label{eqn:opt}
OPT &\le \quant \cdot \tau + \Ex{v_i \in V}{\max_i(0,v_i-\tau)}\\
&\le \quant\cdot\tau+ \sum_{i}\Ex{v_i \in V}{(v_i-\tau)^+}
\end{align}
Next, we present a lower bound for the obtained revenue of uniform
virtual price mechanism. Since it is a sequential posted pricing
mechanism, we consider the worst arrival scenario for the clones. We
set the uniform virtual price equal to $\tau$. Now the lower bound
for the obtained revenue for such mechanism is:
\begin{align}
\label{eqn:apx} \tau\cdot \quant + \sum_i \Ex[v_i\in V]{(v_i
-\tau)^+| \ \forall j \neq i\  v_j<
\tau}\cdot P(\forall j \ v_j < \tau)\\
&\ge \tau \cdot \quant + (1-\quant)\cdot \sum_i \Ex[v_i \in V]{(v_i-\tau)^+}\\
\end{align}
Next we consider $2$ cases:
\begin{itemize}
\item
$\quant \ge \frac{1}{2}$. In this scenario, lemma[9] in \cite{CHK07}
already showed that the uniform virtual price with
$\quant=\frac{1}{2}$ obtains at least half of the optimal with $q=1$
which itself is an upper bound for the optimal solution for any
smaller feasibility constraint $\quant$.
\item
$\quant \le \frac{1}{2}$. In this case, we have $1-\quant \ge
\frac{1}{2}$. Comparing \eqref{eqn:opt}, \eqref{eqn:apx}, we can see
that the uniform virtual price obtains at least half of the optimal
(and in fact the ratio improves as $\quant$ gets smaller). More
accurately, the uniform ironed virtual price obtains
$\max(\frac{1}{2},1-\quant)$ of the optimal solution.
\end{itemize}
\end{proof}
\begin{remark}
Note that Myerson is linear and so is
marginal-uniform-ironed-virtual prices. As a result, showing
\autoref{lemma:copy} is sufficient to show that the marginal uniform
ironed virtual prices is also a $2-$approximation for a given
allocation feasibility constraint: $\qalloc(\quant)$.
\end{remark}
Next, we compare the revenue of the optimal lottery pricing in the
original environment with the optimal revenue of the corresponding
setting in the representative environment in the presence of interim
allocation feasibility constraint.
\begin{lemma}
\label{lemma:lotteryq} For any product distribution $\Dist =
\Dist_1\times\ldots \times\Dist_m$ the expected revenue of optimal
single-agent lottery pricing with the expected probability of
allocation at most $\qalloc(\quant)$ is at most twice of the optimal
auction with expected probability of allocation $\qalloc(\quant)$ in
the representative environment.
\end{lemma}
\begin{proof}
We construct two auctions: $\aucl(\qalloc(q))$ and \emph{allocation
constraint Vickrey mechanism} in the representative environment,
from the given optimal lottery pricing for the original environment
and we show that the total revenue of the two feasible auctions is
at least as much as the revenue of the optimal lottery for the
original environment. Suppose in the original environment, the agent
has type $v=(v_1,\cdot,v_m)$ and suppose the lottery
$l=((q_1,\ldots,q_m),p)$ maximizes her utility. The utility of this
agent at the lottery pricing is defined by $\sum_{i=1}^m v_i\cdot
q_i -p$. Without loss of generality, we assume $v_1 \ge v_2\ge
\ldots\ge v_m$. In the corresponding instance in the representative
environment, we present two truthful auctions that both satisfy the
interim allocation feasibility constraint and we show that the
revenue of the optimal lottery pricing is bounded by the sum of the
revenue of these two auctions. The first auction that we call it
$\aucl(\qalloc(\quant))$, allocates the item to the clone $1$ with
value $v_1$ with probability $\quant_1$ and charge him
$p-\sum_{j\neq 1}v_j\cdot \quant_j$. It is clear that the utility of
the clone $1$ in $\aucl(\qalloc(\quant))$ is exactly equal to the
utility of the single agent in lottery pricing. Since $l$ is the
utility maximizing lottery for the single agent, $\aucl(\cdot)$ will
be incentive compatible. It is also clear that the expected
probability of allocation is no more than the probability of
allocation in $l$ which is bounded by $\qalloc(\quant)$. Next, we
show how to bound the revenue of our auction. The revenue of
$\aucl(\qalloc(\quant))$ is :
\begin{align*}
\Rev{\aucl(\qalloc(\quant))}&= p - \sum_{j \neq 1}q_j\cdot v_j\\
\end{align*}
Our second auction is a variation of Vickrey mechanism. We call it
the allocation-constrained Vickrey mechanism subject to
$\qalloc(q)$. We show that its revenue is higher than $\sum_{j \neq
1}q_j\cdot v_j$ for any set of $q_j$'s corresponding to a feasible
lottery subject to $\qalloc(q)$.
\begin{definition}[Allocation constraint Vickrey  mechanism]
\begin{itemize}
\item
For a given $\Dist$ on the typespace of the clones, compute the
distribution of second highest value and define its mapping to the
quantile space by $F_{(2)}(q)$.
\item Define $q_{(2)}(v_{(2)})$ as the quantile of $v_{(2)}$ with
respect to $F_{(2)}$.
\item Serve $v_{(1)}$ at price $v_{(2)}$ with probability $\qalloc(q_{(2)}(v_{(2)}))$.
\end{itemize}
\end{definition}

First, note that the allocation constrained Vickrey mechanism
satisfies the interim allocation feasibility constraint
$\qalloc(q)$. Next we show that the expected payment of this auction
is at least as much as the expected value of $\sum_{j \neq
1}q_j\cdot v_j$ for any set of $q_j$'s corresponding to a feasible
lottery subject to $\qalloc(q)$. Note that $v_{(2)}\ge v_j, \
\forall j \neq 1$. Also since the lottery satisfies the interim
feasibility constraint, for all possible realization of $v$ with
$v_{(2)}= v_2$, the expected probability of allocation of the
lottery is at most $\qalloc(q_{(2)}(v_{(2)}))$. It is also easy to
verify that this auction is incentive compatible. As a result, the
revenue from the optimal lottery is at most twice the revenue of the
representative environment subject to interim feasibility
constraint.
\end{proof}
\begin{remark}
Conditioned on \autoref{cond:linear-rev}, if we have an $\alpha$
approximation to $\rev(\quant)$, we obtain an $\alpha$ approximation
to the optimal revenue.
\end{remark}


==> related.tex <==
\section{Related Work}
Reductions from multi- to single-agent problems in multi-dimensional mechanism design have been studied by \citet{alaei} and \citet{AFH}. \citet{alaei} considers multi-unit combinatorial auctions and provides constant-approximation reductions to the single agent problem. \citet{AFH} first defined service constrained environments and provided optimal reductions to single-agent problems in matroid settings. Our reduction is to a simpler problem which is computing the revenue curve, whereas \citet{AFH} reduces the problem to maximizing revenue subject to any allocation constraint. \citet{Yan} used correlation gap to prove that sequential pricing is a good approximation to optimal mechanisms in matroid settings for single-dimensional problems. Our work extends the use of correlation gap to multi-dimensional problems. Furthermore, we show that our mechanism can be used to achieve approximations beyond matroid settings, namely downward-closed environments.  

==> sd-example.tex <==
\section{Single-item Auction Example}
\label{s:sd-example}

To illustrate the steps of the marginal revenue approach described in
\autoref{s:intro}, we will instantiate it for the example of selling a
single item to agents with values drawn i.i.d.\@ uniformly from 
$[0,1]$.  In the interest of brevity we will omit
formal justifications.


The optimal lottery pricing for a given ex ante service probability $\exquant$
is to post a take-it-or-leave-it price of $1-\exquant$.  The revenue
from such pricing is the price $1-\exquant$ times the probability
$\exquant$ that it is accepted.  Therefore, the revenue curve is
$\rev(\exquant) = (1-\exquant) \times \exquant$ and the marginal
revenue curve is $\marg(\exquant) = 1 - 2\exquant$.

The optimal lottery for ex ante probability $\exquant$ serves the
agent if her value $\val$ is on $[1-\exquant,1]$.  This is the
strongest $\exquant$ measure of the values from the distribution.
This motivates, in Step~\ref{step:quantile}, mapping value $\val$ to quantile $\quant = 1-\val$.
Importantly, with such a mapping, the distribution over quantiles for a
random type is uniform on $[0,1]$.

For our example of a single-item auction, in Step~\ref{step:feasible}
the surplus of marginal revenue is maximized by selecting for service
the agent with the highest positive marginal revenue (which may serve
no agent if all have negative marginal revenues).

Finally, the appropriate calculation for Step~\ref{step:outcome} in
this example is the following.  All losers have payments equal to
zero.  If there is a winner her payment is calculated as
follows. Consider the minimum quantile $\exquant$ the agent could have
and still be selected as the winner in Step~\ref{step:feasible}.
Charge the agent as if she was offered the optimal pricing for
constraint $\exquant$.  In our example that is price $1-\exquant$.

It is easy to see that for agents with values i.i.d.\@ and uniform on
$[0,1]$, the discussion above is exactly deriving the familiar
second-price auction with reserve $1/2$.  Moreover, for those familiar
with the \citet{M81} derivation of the optimal auction via virtual
values, the composition of the mapping from values to quantiles with the
mapping from quantiles to marginal revenues is equal to Myerson's virtual
value function.


==> sd-proofs.tex <==
\section{Single-dimensional Proofs}
\label{s:single-dimensional-proofs}
\label{s:single-dimensional-proof}


We prove that single-dimensional linear agents are revenue linear.  In
the proof below $\rawrev(\exquant)$ denotes the expected revenue from
posting price $\Val(\exquant)$, i.e., $\rawrev(\exquant) = \exquant
\cdot \Val(\exquant)$.

\begin{proof}[Proof of \autoref{t:sd=>lin}] 
Given the setup in \autoref{sec:single-dimensional} it suffices to upper
bound the optimal revenue by the marginal revenue.  
% Consider the following sequence of steps, the second of which invokes revenue equivalence.  
Suppose we optimize for $\calloc$ and get some (possibly
less restrictive) allocation rule $\qalloc$, then, since any allocation rule weaker than $\qalloc$ is also weaker than $\calloc$,
% , then $\qalloc$ better be a fixed point of $\Rev{\cdot}$; moreover,
\begin{align*}
\Rev{\calloc} &=\Rev{\qalloc}.\\
\intertext{By revenue equivalence, the revenue of any allocation
rule is given by its price-posting revenue curve $\rawrev(\cdot)$, i.e.,}
\Rev{\qalloc} &= \expect[\quant]{-\qalloc'(\quant)\cdot\rawrev(\quant)}.\\
\intertext{But, by definition $\rawrev(\quant) \leq \qrev(\quant)$ for all $\quant$, so this revenue is
upper bounded as,}
\expect[\quant]{-\qalloc'(\quant)\cdot\rawrev(\quant)} &\leq \expect{-\qalloc'(\quant)\cdot\qrev(\quant)} = \expect{\marg(\quant)\cdot\qalloc(\quant)},\\
\intertext{which is
equal to the marginal revenue for $\qalloc$.  Applying integration by
parts,\footnotemark} 
\expect{\marg(\quant)\cdot\qalloc(\quant)} &= \expect{-\marg'(\quant)\cdot\cumalloc(\quant)},\\
\intertext{Because $\cumalloc(\quant) \leq \cumcalloc(\quant)$ for all $\quant$ and ``$-\qrev''(\quant)$'' is non-negative by the concavity of $\qrev(\quant)$, we have}
\expect{-\marg'(\quant)\cdot\cumalloc(\quant)} &\leq 
\expect{\smash{-\marg'(\quant)\cdot\cumcalloc(\quant)}}.\\
\intertext{Integrating by parts (reverse of the above), we have the marginal revenue of $\calloc$. }
\expect{\smash{-\qrev''(\quant)\cdot\cumcalloc(\quant)}} &= \MargRev{\calloc}. 
\end{align*}
%% Hu: footnote has to be done this way in intertext, otherwise it doesn't show.
\footnotetext{The constant terms in this integration by parts are usually zero, if not, they will cancel in the final (reverse) integration by parts.}
We conclude that the revenues are equal as, of course, $\MargRev{\calloc} \leq \Rev{\calloc}$.
\end{proof}


==> test.tex <==
\section{Testing Revenue Linearity}
\label{sec:linear-test}

In this section we present a simple algorithm that tests whether a
given type space and a distribution over it is revenue linear.  By
definition we need only to check the linearity of $\REV(\cdot)$.

Recall that $\REV(\cdot)$ is defined on normalized allocation
functions, which are nondecreasing functions defined on $[0, 1]$.
After discretizing the quantile space to pieces of size $1 / N$, each
such function is a convex combination of $N$ reverse step functions.
The coefficients of these step functions in such a linear
representation sum up to~$1$.  Therefore, $\REV(\cdot)$ can be
equivalently seen as \emph{a concave function defined on the
  $(N-1)$-simplex: $\Delta^N = \{(x_1, \ldots, x_N) \in \mathbb R_+^N
  \mid \sum x_i \leq 1\}$}.  In what follows we will present a general
algorithm that tests the linearity of such a function~$f$.

Let $e_i$ be the vector whose coordinates are~$0$ except the $i$-th
one being~$1$ (the vertices of~$\Delta^N$), and let $P$ be the vector
$(1 / N, \cdots, 1 / N)$.

\begin{definition} 
\label{alg:test-linear}
The \emph{concave linearity test algorithm} runs as follows: test if $f(P) = \sum_{i = 1}^N \frac{1}{N} f(e_i)$;  returns Yes if so, and No otherwise.
\end{definition}

\begin{theorem}
\label{thm:test-linear}
Given that $f$ is concave, the concave linearity test algorithm returns Yes if and only if $f$ is linear.
\end{theorem}

We note that the guaranteed concavity of~$f$ is important for the validity of the algorithm.

\begin{proof}
If $f$ is linear, it is obvious that the algorithm returns Yes.  So we only need to prove the other
direction.  We define a function $g$:
\begin{align}
g(x_1, \ldots, x_N) = f(x_1, \ldots, x_N) - \sum_{i = 1}^N x_i f(e_i).
\notag
\end{align}
Then $g(e_i) = 0$ for each $e_i$.  Notice that $g$ is the difference
between a concave function~$f$ and a linear function, and therefore
$g$ is concave.  Also, given that $g$ is $0$ on every vertex of the
polytope~$\Delta^n$, we have that $g \geq 0$ on $\Delta^n$ by basic
properties of concave functions.  It is easy to see that $f$ is linear
if and only if $g$ is $0$ everywhere on $\Delta^n$.

We show the correctness of the algorithm by induction on~$n$.  When
$n$ is~$2$, $g$ is defined on the line segment $\{(x_1, x_2) \mid x_1
+ x_2 = 1, x_1, x_2 \geq 0\}$, and by basic analysis we know that if
$g(1/2, 1/2) = 0$ and $g$ is concave, then $g$ is constantly~$0$,
which shows that $f$ is linear.  Now suppose the case of $N - 1$ has
been proved, we are going to prove the case of~$N$.  Suppose the
algorithm returns Yes, i.e., $g(P) = 0$, we need to prove that $g$ is
constantly~$0$ on~$\Delta^N$.  We first consider the value of $g$ on
the point $(1 / (N-1), \cdots, 1 / (N-1), 0)$.  This point is colinear
with $e_N$ and $P$, and it lies in $\Delta^{N-1} \times \{0\} \subset
\Delta^N$.  In geometric terms, it is the point where the line that
connects $e_N$ and $P$ meets the face $\{\mathbf x \in \Delta^n \mid
\sum_{i = 1}^{N - 1} x_i = 1\}$.  As we have argued, $g$ is
nonnegative everywhere on~$\Delta^N$.  On the other hand, if $g(1 / (N
- 1), \cdots, 1 / (N - 1), 0) > 0$, by the concavity of~$g$, we will
have
\begin{align*}
\STOC{&}g(P) = g\left( \frac{1}{N}, \cdots, \frac{1}{N} \right) \IFSTOCELSE{\\&\qquad}{&} = g\left( \frac{1}{N} \left(0, \cdots, 0, 1 \right) + \frac{N - 1}{N} \left(\frac{1}{N-1}, \cdots, \frac{1}{N-1}, 0
\right) \right)\\
&\STOC{\qquad}
\geq \frac{1}{N} g(e_N) + \frac{N - 1}{N} g \left(\frac{1}{N-1}, \cdots, \frac{1}{N-1}, 0 \right) > 0,
\end{align*}
which would contradict that $g(P) = 0$.  Therefore, we have $g(1 / (N - 1), \cdots, 1 / (N - 1), 0) =
0$.  By induction, we have that $g$ is constantly~$0$ on $\Delta^{N - 1} \times \{0\}$.  By the same reasoning, $g$ is
constantly~$0$ on all points where at least one coordinate is~$0$.  Now consider any point $\mathbf x = (x_1, \ldots, x_N) \in
\Delta^N$ where $x_i > 0$ for all $i$.  Connect $\mathbf x$ and $P$ and elongate the line in both
directions till they intersect the faces of~$\Delta^n$ at points $\tilde {\mathbf x}$ and~$\hat{\mathbf x}$.
\footnote{Formally, let
$\tilde c$ be $\sup \{c: \mathbf x + c (P - \mathbf x) \in \Delta^N\}$, and let $\tilde {\mathbf x}$ be $\mathbf x + \tilde c (P -
\mathbf x)$.  Similarly, let $\hat c$ be $\inf \{c: \mathbf x + c(P - \mathbf x) \in \Delta^N\}$, and let
$\hat{\mathbf x}$ be $\mathbf x + {\hat c} (P - \mathbf x)$.  Since $\Delta^N$ is a closed set,
$\tilde{\mathbf x}$ and $\hat{\mathbf x}$ are well defined points that are in~$\Delta^N$.}  
Then $\tilde {\mathbf x}$ and $\hat{\mathbf x}$ both have some coordinate that is~$0$, and therefore $g(\tilde
{\mathbf x}) = g(\hat{\mathbf x}) = g(P) = 0$.  Since $g(P)$ lies in the interior of the line segment
connecting $\tilde {\mathbf x}$ and $\hat{\mathbf x}$, by concavity this implies that $g$ is~$0$ for all
points lying on this segment, and hence $g(\mathbf x) = 0$.  Since $\mathbf x$ was an arbitrary point in~$\Delta^N$, we
have shown that $g$ is constantly~$0$ on~$\Delta^N$, and hence $f$ is linear.
\end{proof}

